Combined Tractability of Query Evaluation via Tree Automata and Cycluits (Extended Version)

We investigate parameterizations of both database instances and queries that make query evaluation fixed-parameter tractable in combined complexity. We introduce a new Datalog fragment with stratified negation, intensional-clique-guarded Datalog (ICG-Datalog), with linear-time evaluation on structures of bounded treewidth for programs of bounded rule size. Such programs capture in particular conjunctive queries with simplicial decompositions of bounded width, guarded negation fragment queries of bounded CQ-rank, or two-way regular path queries. Our result proceeds via compilation to alternating two-way automata, whose semantics is defined via cyclic provenance circuits (cycluits) that can be tractably evaluated. Last, we prove that probabilistic query evaluation remains intractable in combined complexity under this parameterization.

==> treedetails.tex <==

\paragraph{Trees}

A \emph{tree} $T$ is an acyclic undirected graph $T = (N,E)$ with set of \emph{nodes} $N$ and set of \emph{edges} $E \subseteq \mathscr{P}_2(N)$.
We will often write $n \in T$ for $n \in N$.

A \emph{directed tree} is a tree $T$ with a distinguished node $r \in T$ called the \emph{root} of $T$.
The edges of a directed tree can then be redefined to be directed, with $(n,m)$ being a directed edge if $\{n,m\}$ was an edge and $n$ is closer to the root than $m$.
When $(n,m) \in E$, we say that $n$ is the (unique) \emph{parent} of $m$ and $m$ is a \emph{child} of $n$.
A node having no child is called a \emph{leaf}. A node that is not a leaf is called \emph{internal}.
A directed tree where every internal node has exactly $2$ children is said \emph{binary full}.\\

Given a finite set of symbols $\Gamma$, a $\Gamma$-\emph{labelled tree} (or $\Gamma$-\emph{tree}) $\la T, \lambda \ra$ is a pair of a tree $T$ and a 
\emph{labelling function} $\lambda : T \to \Gamma$.
A $\Gamma$-\emph{tree} is \emph{directed} if its tree is directed, \emph{finite} if its tree is finite and \emph{binary full} if its tree is.\\





